Paying More Attention to Visual Tokens in Self-Evolving Large Multimodal Models

Recently, self-evolving large multimodal models (LMMs) have received attention for improving visual reasoning in a purely unsupervised setting. However, multi-role self-play and self-consistency reward schemes in existing self-evolving LMMs optimize answer agreement without ensuring the decoder attends to visual content, relying instead on statistical language priors to produce self consistent outputs. This leads to a persistent failure mode we term visual under-conditioning, where the decoder relies on language priors rather than the image during generation, manifesting as insufficient attention to visual tokens. As a result, current self-evolving LMMs struggle on vision--language understanding tasks such as image captioning and visual question answering. To address this, we propose VISE (Visual Invariance Self-Evolution), a purely unsupervised self-evolving framework that directly regularizes the model's visual conditioning policy through two complementary invariance-based rewards: a geometric invariance reward that enforces spatial consistency under known transformations, and a semantic invariance reward that penalizes evidence-agnostic generation by requiring the model to recognize the absence of evidence when predicted regions are perturbed. VISE operates within a single model without specialist roles, external reward models, or annotations, and is trained on raw unlabeled images. Experiments on 18 benchmarks demonstrate the efficacy of our approach. Using Qwen3-VL-2B as the base model, VISE achieves gains of $+16.85$ CIDEr on COCO and $+19.66$ CIDEr on TextCaps, reduces object hallucination by $5.0$ Chair-I points, and generalizes across four model families and scales. Our code and models are available at https://mbzuai-oryx.github.io/VISE

==> tables/table6.tex <==
\begin{table}[t]
\centering
\caption{Comparison of \textbf{VISE} against baselines on referring expression grounding benchmarks.
\textcolor{deltaup}{Green}/\textcolor{deltadn}{red} deltas show absolute change relative to base model.}
\label{tab:grounding}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l cc cc cc cc cc}
\toprule
\multirow{2}{*}{\textbf{Method}}
  & \multicolumn{6}{c}{\textbf{RefCOCO+}}
  & \multicolumn{4}{c}{\textbf{RefCOCOg}} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-11}
  & \multicolumn{2}{c}{val}
  & \multicolumn{2}{c}{testA}
  & \multicolumn{2}{c}{testB}
  & \multicolumn{2}{c}{val}
  & \multicolumn{2}{c}{test} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
  & cIoU & GIoU & cIoU & GIoU & cIoU & GIoU & cIoU & GIoU & cIoU & GIoU \\
\midrule

\multicolumn{11}{l}{\textit{Qwen3-VL-2B-Instruct}} \\
\hdashline
Base
& 69.17 & 70.59
& 74.85 & 77.14
& 60.59 & 64.09
& 74.96 & 76.34
& 75.57 & 76.26 \\
VisPlay
& 66.52\dn{2.65} &
67.91\dn{2.68}
& 72.24\dn{2.61} & 73.73\dn{3.41}
& 58.83\dn{1.76} & 62.67\dn{1.42}
& 72.38\dn{2.58} & 74.76\dn{1.58}
& 73.86\dn{1.71} & 74.89\dn{1.37} \\
VisionZero-CLEVR
& 67.84\dn{1.33} & 68.26\dn{2.33}
& 73.76\dn{1.09} & 75.79\dn{1.35}
& 59.18\dn{1.41} & 62.94\dn{1.15}
& 74.18\dn{0.78} & 75.01\dn{1.33}
& 74.69\dn{0.88} & 75.38\dn{0.88} \\
VisionZero-Chart
& 67.89\dn{1.28} & 67.31\dn{3.28}
& 73.58\dn{1.27} & 73.64\dn{3.50}
& 59.25\dn{1.34} & 62.97\dn{1.12}
& 73.23\dn{1.73} & 75.08\dn{1.26}
& 74.21\dn{1.36} & 75.14\dn{1.12} \\
VisionZero-RW
& 68.06\dn{1.11} & 69.17\dn{1.42}
& 74.58\dn{0.27} & 75.92\dn{1.22}
& 59.81\dn{0.78} & 63.01\dn{1.08}
& 74.69\dn{0.27} & 75.12\dn{1.22}
& 75.84\up{0.27} & 76.31\up{0.05} \\
EvoLMM
& 67.19\dn{1.98} & 69.41\dn{1.18}
& 73.39\dn{1.46} & 75.16\dn{1.98}
& 59.45\dn{1.14} & 62.91\dn{1.18}
& 73.98\dn{0.98} & 74.96\dn{1.38}
& 74.12\dn{1.45} & 75.57\dn{0.69} \\
iReasoner
& 67.22\dn{1.95} & 69.43\dn{1.16}
& 73.42\dn{1.43} & 75.19\dn{1.95}
& 59.49\dn{1.10} & 62.96\dn{1.13}
& 74.02\dn{0.94} & 75.04\dn{1.30}
& 74.16\dn{1.41} & 75.59\dn{0.67} \\
\rowcolor{rowblue}
\textbf{Ours}
& 68.29\dn{0.88} & 70.52\dn{0.07}
& 74.68\dn{0.17} & 76.27\dn{0.87}
& 60.41\dn{0.18} & 63.86\dn{0.23}
& 75.35\up{0.39}  & 76.56\up{0.22}
& 75.66\up{0.09}  & 76.58\up{0.32} \\

\midrule

\multicolumn{11}{l}{\textit{Qwen3-VL-4B-Instruct}} \\
\hdashline

Base
& 77.43 & 79.02 & 82.01 & 83.31 & 70.14 & 73.21 & 79.22 & 80.67 & 79.18 & 80.36 \\
VisPlay
& 76.97\dn{0.46} & 78.27\dn{0.75} & 81.39\dn{0.62} & 82.68\dn{0.63} & 69.18\dn{0.96} & 72.19\dn{1.02} & 78.96\dn{0.26} & 80.28\dn{0.39} & 78.89\dn{0.29} & 80.01\dn{0.35} \\
VisionZero-CLEVR
& 77.03\dn{0.40} & 78.42\dn{0.60} & 81.56\dn{0.45} & 82.81\dn{0.50} & 69.32\dn{0.82} & 72.35\dn{0.86} & 79.07\dn{0.15} & 80.43\dn{0.24} & 79.06\dn{0.12} & 80.17\dn{0.19} \\
VisionZero-Chart
& 77.16\dn{0.27} & 78.53\dn{0.49} & 81.65\dn{0.36} & 82.92\dn{0.39} & 69.43\dn{0.71} & 72.44\dn{0.77} & 79.18\dn{0.04} & 80.49\dn{0.18} & 79.08\dn{0.10}  & 80.24\dn{0.12} \\
VisionZero-RW
& 77.23\dn{0.20} & 78.62\dn{0.40} & 81.78\dn{0.23} & 83.09\dn{0.22} & 69.57\dn{0.57} & 72.56\dn{0.65} & 79.23\up{0.01} & 80.63\dn{0.04} & 79.21\up{0.03} & 80.28\dn{0.08} \\
EvoLMM
& 77.10\dn{0.33} & 78.46\dn{0.56} & 81.61\dn{0.40} & 82.85\dn{0.46} & 69.37\dn{0.77} & 72.36\dn{0.85} & 79.10\dn{0.12} & 80.41\dn{0.26} & 79.11\dn{0.07} & 80.19\dn{0.17} \\
iReasoner
& 77.14\dn{0.29} & 78.50\dn{0.52} & 81.63\dn{0.38} & 82.89\dn{0.42} & 69.38\dn{0.76} & 72.42\dn{0.79} & 79.14\dn{0.08} & 80.47\dn{0.20} & 79.13\dn{0.05} & 80.22\dn{0.14} \\
\rowcolor{rowblue}
\textbf{Ours}
& 77.33\dn{0.10} & 78.78\dn{0.24} & 81.88\dn{0.13} & 83.12\dn{0.19} & 69.68\dn{0.46} & 72.65\dn{0.56} & 79.36\up{0.14} & 80.78\up{0.11} & 79.33\up{0.15} & 80.39\up{0.03} \\

\bottomrule
\end{tabular}%
}
\end{table}

